Quench Spectroscopy for Dissipative and (Non)-Hermitian Quantum Lattice Models

We extend the quench spectroscopy method to dissipative and isolated non-Hermitian quantum lattice models via the case study of the open Bose-Hubbard chain and the non-Hermitian transverse-field Ising chain respectively. We first investigate theoretically the dynamics of the open Bose-Hubbard chain confined in the superfluid phase induced by a sudden global quench on the dissipations and the repulsive interactions using the equation-of-motion approach. Using the same analytical approach, we then discuss the applicability of the quench spectroscopy to non-Hermitian quantum lattice models by considering the sudden global quench dynamics of the non-Hermitian transverse-field Ising chain confined in the paramagnetic phase. We finally generalize this spectroscopy method to isolated Hermitian quantum lattice models characterized by a quadratic fermionic or bosonic Hamiltonian. For this purpose, we consider the case study of the Hermitian version of the latter one-dimensional lattice model. The investigation is performed analytically for the bosonic and fermionic reformulations while considering for each case the equation-of-motion and quasiparticle theoretical approaches.

==> journalsVaps.tex <==
\newcommand{\Jnature}{Nature (London)}
\newcommand{\Jnatphys}{Nat. Phys.}
\newcommand{\Jnatcomm}{Nat. Comm.}
\newcommand{\Jnatmat}{Nat. Mater.}
\newcommand{\JSciRep}{Sci. Rep.}

\newcommand{\Jscience}{Science}

\newcommand{\Jprx}{Phys. Rev. X}
\newcommand{\Jprl}{Phys. Rev. Lett.}
\newcommand{\Jpr}{Phys. Rev.}
\newcommand{\Jpra}{Phys. Rev. A}
\newcommand{\Jprb}{Phys. Rev. B}
\newcommand{\Jprc}{Phys. Rev. C}
\newcommand{\Jprd}{Phys. Rev. D}
\newcommand{\Jpre}{Phys. Rev. E}
\newcommand{\Jrmp}{Rev. Mod. Phys.}

\newcommand{\JplA}{Phys. Lett. A}

\newcommand{\Jepl}{Europhys. Lett.}
\newcommand{\Jnjp}{New J. Phys.}
\newcommand{\Jepjb}{Eur. Phys. J. B}
\newcommand{\Jepjd}{Eur. Phys. J. D}
\newcommand{\Jepjst}{Eur. Phys. J. Special Topics}

\newcommand{\Jjosab}{J. Opt. Soc. Am. B}
\newcommand{\JApplPhysLett}{Appl. Phys. Lett.}
\newcommand{\JApplPhysB}{Appl. Phys. B}

\newcommand{\Joptcomm}{Opt. Comm.}
\newcommand{\JApplOpt}{Appl. Opt.}

\newcommand{\JphysA}{J. Phys. A}

\newcommand{\JphyslettA}{J. Phys. Lett. A}
\newcommand{\JphyslettB}{J. Phys. Lett. B}

\newcommand{\JnulcphysA}{Nucl. Phys. A}

\newcommand{\Jbullamphyssoc}{Bull. Am. Phys. Soc.}

\newcommand{\Jphysjap}{J. Phys. Soc. Japan}

\newcommand{\JJlowT}{J. Low Temp. Phys.}

\newcommand{\Jprocroysoc}{Proc. Roy. Soc. A: Math. Phys. Eng. Sci.}

\newcommand{\Jjetp}{Sov. Phys. JETP}
\newcommand{\Jjetplett}{JETP Lett.}
\newcommand{\JjphysUSSR}{J. Phys. USSR}
\newcommand{\JSovJlowT}{Sov. J. Low Temp. Phys.}

\newcommand{\JZhEkspTeorFiz}{Zh. Eksp. Teor. Fiz.}

\newcommand{\Jjchemphys}{J. Chem. Phys.}
\newcommand{\Jjphyschemsol}{J. Phys. Chem. Sol.}
\newcommand{\Jsolstatecomm}{Solid State Comm.}

\newcommand{\Jijmpb}{Int. J. Mod. Phys. B}

\newcommand{\Jijthphys}{Int. J. Theor. Phys.}

\newcommand{\JphysicaB}{Physica B}
\newcommand{\JphysicaBC}{Physica B+C}

\newcommand{\Jstatmech}{J. Stat. Mech.}

\newcommand{\Jphysrep}{Phys. Rep.}
\newcommand{\JRepProgPhys}{Rep. Prog. Phys.}
\newcommand{\JjphysCM}{J. Phys.: Cond. Matt.}
\newcommand{\JjphysA}{J. Phys. A: Math. Theor.}
\newcommand{\JjphysB}{J. Phys. B: At. Mol. Opt. Phys.}
\newcommand{\JjphysC}{J. Phys. C: Solid State Phys.}
\newcommand{\JjphysF}{J. Phys. F: Metal Phys.}
\newcommand{\Jphystoday}{Phys. Today}

\newcommand{\Jadvphys}{Adv. Phys.}

\newcommand{\Jannphys}{Ann. Phys. (NY)}

\newcommand{\JAnnualRevCondMat}{Annual Rev. Cond. Mat. Phys.}

\newcommand{\Jadvatmoloptphys}{Adv. At. Mol. Opt. Phys.}
\newcommand{\Joptexpr}{Opt. Express}

\newcommand{\JphysB}{J. Phys. B: At. Mol. Opt. Phys.}

\newcommand{\JTheorMathPhys}{Theor. Math. Phys.}
\newcommand{\JMathPhys}{J. Math. Phys.}
\newcommand{\JCommMathPhys}{Comm. Math. Phys.}

\newcommand{\Jprogthphys}{Prog. Theor. Phys.}
\newcommand{\Jprogthphyssup}{Prog. Theor. Phys., Suppl.}

\newcommand{\JjphysFr}{J. Phys. (France)}
\newcommand{\JjphysquatreF}{J. Phys. IV (France)}

\newcommand{\Jcommmathphys}{Comm. Math. Phys.}

\newcommand{\JZphysB}{Z. Phys. B}
